Stellar surface information from the Ca II H&K lines I. Intensity profiles of the solar activity components

The detection of Earth-like planets with the radial-velocity method is currently limited by the presence of stellar activity signatures. On rotational timescales, spots and plages (or faculae) are known to introduce different RV signals, but their corrections require better activity proxies. The best-known chromospheric activity proxies in the visible are the Ca II H & K lines, but the physical quantities measured by their profiles need to be clarified. We first investigate resolved images of the Sun in order to better understand the spectrum of plages, spots, and the network using the Meudon spectroheliogram. We show that distinct line profiles are produced by plages, spots, and by the network component and we also derived the center-to-limb variations of the three profiles. Some care is required to disentangle their contributions due to their similarities. By combining disk-integrated spectra from the ISS high-resolution spectrograph with SDO direct images of the Sun, we managed to extract a high-resolution emission spectrum of the different components, which tend to confirm the spectra extracted from the Meudon spectroheliogram datacubes. Similar results were obtained with the HARPS-N Sun-as-a-star spectra. We concluded using a three-component model that the temporal variation of the popular S-index contains, on average for the 24th solar cycle: 70 +/- 12% of plage, 26 +/- 12% of network and 4 +/- 4% of spots. This preliminary investigation suggests that a detailed study of the Ca II H & K profiles may provide rich information about the filling factor and distribution of different types of active regions.

==> CDS/YAMORI1/ReadMe <==
                                                      (M.Cretignier, 2023)
================================================================================
Stellar surface information from the Ca II H&K lines. I. Intensity profiles of
the solar activity components
    M.Cretignier, A.G.M Pietrow, S.Aigrain
    =References ?
================================================================================
Keywords: exoplanets – stars: activity – stars: chromospheres –
          methods: data analysis – techniques: spectroscopic

Abstract:
        The detection of Earth-like planets with the radial-velocity method is
  currently limited by the presence of stellar activity     signatures. On
  rotational timescales, spots and plages (or faculae) are known to introduce
  different RV signals, but their     corrections require better activity
  proxies. The best-known chromospheric activity proxies in the visible are the
  Ca II H & K     lines, but the physical quantities measured by their profiles
  need to be clarified. We first investigate resolved images of the Sun     in
  order to better understand the spectrum of plages, spots, and the network
  using the Meudon spectroheliogram. We show     that distinct line profiles are
  produced by plages, spots, and by the network component and we also derived
  the center-to-limb     variations of the three profiles. Some care is required
  to disentangle their contributions due to their similarities. By combining
  disk-integrated spectra from the ISS high-resolution spectrograph with SDO
  direct images of the Sun, we managed to extract a     high-resolution emission
  spectrum of the different components, which tend to confirm the spectra
  extracted from the Meudon     spectroheliogram datacubes. Similar results were
  obtained with the HARPS-N Sun-as-a-star spectra. We concluded using a
  three-component model that the temporal variation of the popular 𝑆index
  contains, on average for the 24th solar cycle: 70 ± 12\%     of plage, 26 ±
  12\% of network and 4 ± 4\% of spots. This preliminary investigation suggests
  that a detailed study of the Ca II H     & K profiles may provide rich
  information about the filling factor and distribution of different types of
  active regions.

Description:
       CLV spectra for Ca II H&K lines for spots, plage and quiet Sun obtained
  with the Meudon spectroheliograms from Cretignier et al. 2023

File Summary:
--------------------------------------------------------------------------------
 FileName    Lrecl   Records    Explanations
--------------------------------------------------------------------------------
ReadMe          80        .  this file
quiet.cds      110       94  CSV table of CLV profiles for quiet Sun
spot.cds        74       94  CSV table of CLV profiles for spot Sun
plage.cds       74       94  CSV table of CLV profiles for plage Sun


--------------------------------------------------------------------------------
Byte-by-byte Description of file: quiet.cds
--------------------------------------------------------------------------------
 Bytes Format Units  Label     Explanations
--------------------------------------------------------------------------------
  1-  2   I2     ---    index         Index of the table
  4- 11   F8.4   nm     wave          Wavelength        
 13- 20   F8.6   %      flux_0.078    Flux at mu=0.078  
 22- 30   F9.6   %      flux_0.156    Flux at mu=0.156  
 32- 40   F9.6   %      flux_0.253    Flux at mu=0.253  
 42- 50   F9.6   %      flux_0.353    Flux at mu=0.353  
 52- 60   F9.6   %      flux_0.452    Flux at mu=0.452  
 62- 70   F9.6   %      flux_0.552    Flux at mu=0.552  
 72- 80   F9.6   %      flux_0.646    Flux at mu=0.646  
 82- 90   F9.6   %      flux_0.751    Flux at mu=0.751  
 92-100   F9.6   %      flux_0.846    Flux at mu=0.846  
102-110   F9.6   %      flux_0.946    Flux at mu=0.946  

--------------------------------------------------------------------------------

Byte-by-byte Description of file: spot.cds
--------------------------------------------------------------------------------
 Bytes Format Units  Label     Explanations
--------------------------------------------------------------------------------
 1- 2   I2     ---    index         Index of the table               
 4-11   F8.4   nm     wave          Wavelength                       
13-20   F8.6   ---    flux_0.353    Flux ratio (AR/Quiet) at mu=0.353
22-29   F8.6   ---    flux_0.459    Flux ratio (AR/Quiet) at mu=0.459
31-38   F8.6   ---    flux_0.551    Flux ratio (AR/Quiet) at mu=0.551
40-47   F8.6   ---    flux_0.650    Flux ratio (AR/Quiet) at mu=0.650
49-56   F8.6   ---    flux_0.758    Flux ratio (AR/Quiet) at mu=0.758
58-65   F8.6   ---    flux_0.860    Flux ratio (AR/Quiet) at mu=0.860
67-74   F8.6   ---    flux_0.941    Flux ratio (AR/Quiet) at mu=0.941

--------------------------------------------------------------------------------

Byte-by-byte Description of file: plage.cds
--------------------------------------------------------------------------------
 Bytes Format Units  Label     Explanations
--------------------------------------------------------------------------------
 1- 2   I2     ---    index         Index of the table               
 4-11   F8.4   nm     wave          Wavelength                       
13-20   F8.6   ---    flux_0.352    Flux ratio (AR/Quiet) at mu=0.352
22-29   F8.6   ---    flux_0.454    Flux ratio (AR/Quiet) at mu=0.454
31-38   F8.6   ---    flux_0.553    Flux ratio (AR/Quiet) at mu=0.553
40-47   F8.6   ---    flux_0.651    Flux ratio (AR/Quiet) at mu=0.651
49-56   F8.6   ---    flux_0.753    Flux ratio (AR/Quiet) at mu=0.753
58-65   F8.6   ---    flux_0.856    Flux ratio (AR/Quiet) at mu=0.856
67-74   F8.6   ---    flux_0.940    Flux ratio (AR/Quiet) at mu=0.940

--------------------------------------------------------------------------------



See also:
 https://ui.adsabs... : Cretignier et al. 2023


Acknowledgements:

References:
================================================================================
     (prepared by author  / pyreadme )


==> CDS/YAMORI1/ReadMe2 <==
                                                      (M.Cretignier, 2023)
================================================================================
Stellar surface information from the Ca II H&K lines. I. Intensity profiles of
the solar activity components
    M.Cretignier, A.G.M Pietrow, S.Aigrain
    =References ?
================================================================================
Keywords: exoplanets – stars: activity – stars: chromospheres –
          methods: data analysis – techniques: spectroscopic

Objects:
    -----------------------------------------
       RA   (2000)   DE    Designation(s)
    -----------------------------------------

Abstract:
        The detection of Earth-like planets with the radial-velocity method is
  currently limited by the presence of stellar activity     signatures. On
  rotational timescales, spots and plages (or faculae) are known to introduce
  different RV signals, but their     corrections require better activity
  proxies. The best-known chromospheric activity proxies in the visible are the
  Ca II H & K     lines, but the physical quantities measured by their profiles
  need to be clarified. We first investigate resolved images of the Sun     in
  order to better understand the spectrum of plages, spots, and the network
  using the Meudon spectroheliogram. We show     that distinct line profiles are
  produced by plages, spots, and by the network component and we also derived
  the center-to-limb     variations of the three profiles. Some care is required
  to disentangle their contributions due to their similarities. By combining
  disk-integrated spectra from the ISS high-resolution spectrograph with SDO
  direct images of the Sun, we managed to extract a     high-resolution emission
  spectrum of the different components, which tend to confirm the spectra
  extracted from the Meudon     spectroheliogram datacubes. Similar results were
  obtained with the HARPS-N Sun-as-a-star spectra. We concluded using a
  three-component model that the temporal variation of the popular 𝑆index
  contains, on average for the 24th solar cycle: 70 ± 12\%     of plage, 26 ±
  12\% of network and 4 ± 4\% of spots. This preliminary investigation suggests
  that a detailed study of the Ca II H     & K profiles may provide rich
  information about the filling factor and distribution of different types of
  active regions.

Description:
       CLV spectra for Ca II H&K lines for spots, plage and quiet Sun obtained
  with the Meudon spectroheliograms from Cretignier et al. 2023

File Summary:
--------------------------------------------------------------------------------
 FileName    Lrecl   Records    Explanations
--------------------------------------------------------------------------------
ReadMe          80        .  this file
quiet.cds      110       94  CSV table of CLV profiles for quiet Sun
spot.cds        74       94  CSV table of CLV profiles for spot Sun
plage.cds       74       94  CSV table of CLV profiles for plage Sun


--------------------------------------------------------------------------------
Byte-by-byte Description of file: quiet.cds
--------------------------------------------------------------------------------
 Bytes Format Units  Label     Explanations
--------------------------------------------------------------------------------
  1-  2   I2     ---    index       Description of index
  4- 11   F8.4   ---    wave       [392.92/393.81] Description of wave
 13- 20   F8.6   ---    flux_0.078 [2.09/6.09] Description of flux_0.078
 22- 30   F9.6   ---    flux_0.156 [2.6/11.49] Description of flux_0.156
 32- 40   F9.6   ---    flux_0.253 [3.23/15.25] Description of flux_0.253
 42- 50   F9.6   ---    flux_0.353 [4.16/17.84] Description of flux_0.353
 52- 60   F9.6   ---    flux_0.452 [4.56/19.88] Description of flux_0.452
 62- 70   F9.6   ---    flux_0.552 [4.92/22.08] Description of flux_0.552
 72- 80   F9.6   ---    flux_0.646 [5.26/24.36] Description of flux_0.646
 82- 90   F9.6   ---    flux_0.751 [5.69/27.13] Description of flux_0.751
 92-100   F9.6   ---    flux_0.846 [6.05/29.73] Description of flux_0.846
102-110   F9.6   ---    flux_0.946 [6.32/32.75] Description of flux_0.946

--------------------------------------------------------------------------------

Byte-by-byte Description of file: spot.cds
--------------------------------------------------------------------------------
 Bytes Format Units  Label     Explanations
--------------------------------------------------------------------------------
 1- 2   I2     ---    index       Description of index
 4-11   F8.4   ---    wave       [392.92/393.81] Description of wave
13-20   F8.6   ---    flux_0.353 [0.51/2.53] Description of flux_0.353
22-29   F8.6   ---    flux_0.459 [0.58/2.29] Description of flux_0.459
31-38   F8.6   ---    flux_0.551 [0.59/2.9] Description of flux_0.551
40-47   F8.6   ---    flux_0.650 [0.57/2.45] Description of flux_0.650
49-56   F8.6   ---    flux_0.758 [0.57/2.45] Description of flux_0.758
58-65   F8.6   ---    flux_0.860 [0.58/2.33] Description of flux_0.860
67-74   F8.6   ---    flux_0.941 [0.59/2.05] Description of flux_0.941

--------------------------------------------------------------------------------

Byte-by-byte Description of file: plage.cds
--------------------------------------------------------------------------------
 Bytes Format Units  Label     Explanations
--------------------------------------------------------------------------------
 1- 2   I2     ---    index       Description of index
 4-11   F8.4   ---    wave       [392.92/393.81] Description of wave
13-20   F8.6   ---    flux_0.352 [1.05/3.57] Description of flux_0.352
22-29   F8.6   ---    flux_0.454 [1.06/3.38] Description of flux_0.454
31-38   F8.6   ---    flux_0.553 [1.08/3.47] Description of flux_0.553
40-47   F8.6   ---    flux_0.651 [1.09/3.37] Description of flux_0.651
49-56   F8.6   ---    flux_0.753 [1.09/3.31] Description of flux_0.753
58-65   F8.6   ---    flux_0.856 [1.09/3.24] Description of flux_0.856
67-74   F8.6   ---    flux_0.940 [1.09/3.3] Description of flux_0.940

--------------------------------------------------------------------------------



See also:
 https://ui.adsabs... : Cretignier et al. 2023


Acknowledgements:

References:
================================================================================
     (prepared by author  / pyreadme )

